Geometry Error Analysis of a parametric mapping for Higher Order Unfitted Space-Time Methods

In [Heimann, Lehrenfeld, Preu{\ss}, SIAM J. Sci. Comp. 45(2), 2023, B139 - B165] new geometrically unfitted space-time Finite Element methods for partial differential equations posed on moving domains of higher-order accuracy in space and time have been introduced. For geometrically higher-order accuracy a parametric mapping on a background space-time tensor-product mesh has been used. In this paper, we concentrate on the geometrical accuracy of the approximation and derive rigorous bounds for the distance between the realized and an ideal mapping in different norms and derive results for the space-time regularity of the parametric mapping. These results are important and lay the ground for the error analysis of corresponding unfitted space-time finite element methods.

==> num_exp/comp_tableK_k1.tex <==
1 & 0 & $7.09\!\cdot\!10^{-1}$ &  & $1.8\!\cdot\!10^{-1}$ & $6.57\!\cdot\!10^{-1}$ &  & $4.7\!\cdot\!10^{-3}$ & $6.56\!\cdot\!10^{-1}$ &  & $2.4\!\cdot\!10^{-5}$\\ 
 & 1 & $2.05\!\cdot\!10^{-1}$ & \scriptsize\texttt{(1.8)}\normalsize & $1.8\!\cdot\!10^{-2}$ & $2.06\!\cdot\!10^{-1}$ & \scriptsize\texttt{(1.7)}\normalsize & $1.2\!\cdot\!10^{-3}$ & $2.06\!\cdot\!10^{-1}$ & \scriptsize\texttt{(1.7)}\normalsize & $1.5\!\cdot\!10^{-5}$\\ 
 & 2 & $5.55\!\cdot\!10^{-2}$ & \scriptsize\texttt{(1.9)}\normalsize & $4.2\!\cdot\!10^{-4}$ & $5.55\!\cdot\!10^{-2}$ & \scriptsize\texttt{(1.9)}\normalsize & $8.8\!\cdot\!10^{-5}$ & $5.55\!\cdot\!10^{-2}$ & \scriptsize\texttt{(1.9)}\normalsize & $1.2\!\cdot\!10^{-6}$\\ 
 & 3 & $1.51\!\cdot\!10^{-2}$ & \scriptsize\texttt{(1.9)}\normalsize & $2.8\!\cdot\!10^{-4}$ & $1.51\!\cdot\!10^{-2}$ & \scriptsize\texttt{(1.9)}\normalsize & $4.3\!\cdot\!10^{-6}$ & $1.51\!\cdot\!10^{-2}$ & \scriptsize\texttt{(1.9)}\normalsize & $7.6\!\cdot\!10^{-8}$\\ 
 & 4 & $3.89\!\cdot\!10^{-3}$ & \scriptsize\texttt{(2.0)}\normalsize & $9.9\!\cdot\!10^{-6}$ & $3.89\!\cdot\!10^{-3}$ & \scriptsize\texttt{(2.0)}\normalsize & $5.3\!\cdot\!10^{-6}$ & $3.89\!\cdot\!10^{-3}$ & \scriptsize\texttt{(2.0)}\normalsize & $6.2\!\cdot\!10^{-8}$\\ 
 & 5 & $9.76\!\cdot\!10^{-4}$ & \scriptsize\texttt{(2.0)}\normalsize & $9.0\!\cdot\!10^{-6}$ & $9.76\!\cdot\!10^{-4}$ & \scriptsize\texttt{(2.0)}\normalsize & $3.4\!\cdot\!10^{-7}$ & $9.76\!\cdot\!10^{-4}$ & \scriptsize\texttt{(2.0)}\normalsize & $5.1\!\cdot\!10^{-9}$\\ 
 & 6 & $2.46\!\cdot\!10^{-4}$ & \scriptsize\texttt{(2.0)}\normalsize & $7.1\!\cdot\!10^{-8}$ & $2.46\!\cdot\!10^{-4}$ & \scriptsize\texttt{(2.0)}\normalsize & $1.4\!\cdot\!10^{-7}$ & $2.46\!\cdot\!10^{-4}$ & \scriptsize\texttt{(2.0)}\normalsize & $1.4\!\cdot\!10^{-9}$\\ 


==> num_exp/comp_tableK_k2.tex <==
2 & 0 & $5.42\!\cdot\!10^{-1}$ &  & $6.4\!\cdot\!10^{-3}$ & $5.44\!\cdot\!10^{-1}$ &  & $6.1\!\cdot\!10^{-3}$ & $5.43\!\cdot\!10^{-1}$ &  & $7.4\!\cdot\!10^{-5}$\\ 
 & 1 & $2.03\!\cdot\!10^{-2}$ & \scriptsize\texttt{(4.7)}\normalsize & $4.5\!\cdot\!10^{-3}$ & $2.01\!\cdot\!10^{-2}$ & \scriptsize\texttt{(4.8)}\normalsize & $4.4\!\cdot\!10^{-4}$ & $2.01\!\cdot\!10^{-2}$ & \scriptsize\texttt{(4.8)}\normalsize & $5.4\!\cdot\!10^{-6}$\\ 
 & 2 & $2.32\!\cdot\!10^{-3}$ & \scriptsize\texttt{(3.1)}\normalsize & $2.5\!\cdot\!10^{-4}$ & $2.32\!\cdot\!10^{-3}$ & \scriptsize\texttt{(3.1)}\normalsize & $2.0\!\cdot\!10^{-5}$ & $2.32\!\cdot\!10^{-3}$ & \scriptsize\texttt{(3.1)}\normalsize & $2.2\!\cdot\!10^{-7}$\\ 
 & 3 & $3.13\!\cdot\!10^{-4}$ & \scriptsize\texttt{(2.9)}\normalsize & $6.2\!\cdot\!10^{-6}$ & $3.13\!\cdot\!10^{-4}$ & \scriptsize\texttt{(2.9)}\normalsize & $1.3\!\cdot\!10^{-6}$ & $3.13\!\cdot\!10^{-4}$ & \scriptsize\texttt{(2.9)}\normalsize & $1.6\!\cdot\!10^{-8}$\\ 
 & 4 & $3.84\!\cdot\!10^{-5}$ & \scriptsize\texttt{(3.0)}\normalsize & $2.3\!\cdot\!10^{-6}$ & $3.84\!\cdot\!10^{-5}$ & \scriptsize\texttt{(3.0)}\normalsize & $5.0\!\cdot\!10^{-8}$ & $3.84\!\cdot\!10^{-5}$ & \scriptsize\texttt{(3.0)}\normalsize & $7.7\!\cdot\!10^{-10}$\\ 
 & 5 & $4.76\!\cdot\!10^{-6}$ & \scriptsize\texttt{(3.0)}\normalsize & $2.0\!\cdot\!10^{-7}$ & $4.75\!\cdot\!10^{-6}$ & \scriptsize\texttt{(3.0)}\normalsize & $1.2\!\cdot\!10^{-8}$ & $4.75\!\cdot\!10^{-6}$ & \scriptsize\texttt{(3.0)}\normalsize & $1.5\!\cdot\!10^{-10}$\\ 
 & 6 & $5.94\!\cdot\!10^{-7}$ & \scriptsize\texttt{(3.0)}\normalsize & $1.3\!\cdot\!10^{-8}$ & $5.93\!\cdot\!10^{-7}$ & \scriptsize\texttt{(3.0)}\normalsize & $1.3\!\cdot\!10^{-10}$ & $5.93\!\cdot\!10^{-7}$ & \scriptsize\texttt{(3.0)}\normalsize & $4.9\!\cdot\!10^{-12}$\\ 


==> num_exp/comp_tableK_k3.tex <==
3 & 0 & $3.27\!\cdot\!10^{-1}$ &  & $9.8\!\cdot\!10^{-2}$ & $3.39\!\cdot\!10^{-1}$ &  & $7.5\!\cdot\!10^{-3}$ & $3.40\!\cdot\!10^{-1}$ &  & $7.5\!\cdot\!10^{-5}$\\ 
 & 1 & $3.59\!\cdot\!10^{-3}$ & \scriptsize\texttt{(6.5)}\normalsize & $2.6\!\cdot\!10^{-3}$ & $2.95\!\cdot\!10^{-3}$ & \scriptsize\texttt{(6.8)}\normalsize & $3.1\!\cdot\!10^{-4}$ & $2.90\!\cdot\!10^{-3}$ & \scriptsize\texttt{(6.9)}\normalsize & $3.5\!\cdot\!10^{-6}$\\ 
 & 2 & $1.97\!\cdot\!10^{-4}$ & \scriptsize\texttt{(4.2)}\normalsize & $1.2\!\cdot\!10^{-4}$ & $1.64\!\cdot\!10^{-4}$ & \scriptsize\texttt{(4.2)}\normalsize & $7.3\!\cdot\!10^{-6}$ & $1.62\!\cdot\!10^{-4}$ & \scriptsize\texttt{(4.2)}\normalsize & $8.0\!\cdot\!10^{-8}$\\ 
 & 3 & $1.03\!\cdot\!10^{-5}$ & \scriptsize\texttt{(4.3)}\normalsize & $8.0\!\cdot\!10^{-6}$ & $8.64\!\cdot\!10^{-6}$ & \scriptsize\texttt{(4.2)}\normalsize & $2.7\!\cdot\!10^{-7}$ & $8.61\!\cdot\!10^{-6}$ & \scriptsize\texttt{(4.2)}\normalsize & $2.9\!\cdot\!10^{-9}$\\ 
 & 4 & $6.76\!\cdot\!10^{-7}$ & \scriptsize\texttt{(3.9)}\normalsize & $4.6\!\cdot\!10^{-7}$ & $5.63\!\cdot\!10^{-7}$ & \scriptsize\texttt{(3.9)}\normalsize & $9.6\!\cdot\!10^{-9}$ & $5.62\!\cdot\!10^{-7}$ & \scriptsize\texttt{(3.9)}\normalsize & $9.9\!\cdot\!10^{-11}$\\ 
 & 5 & $4.08\!\cdot\!10^{-8}$ & \scriptsize\texttt{(4.1)}\normalsize & $2.6\!\cdot\!10^{-8}$ & $3.43\!\cdot\!10^{-8}$ & \scriptsize\texttt{(4.0)}\normalsize & $3.7\!\cdot\!10^{-10}$ & $3.42\!\cdot\!10^{-8}$ & \scriptsize\texttt{(4.0)}\normalsize & $4.5\!\cdot\!10^{-12}$\\ 


==> num_exp/comp_tableK_k4.tex <==
4 & 0 & $4.50\!\cdot\!10^{-1}$ &  & $2.7\!\cdot\!10^{-1}$ & $5.20\!\cdot\!10^{-1}$ &  & $5.0\!\cdot\!10^{-2}$ & $5.38\!\cdot\!10^{-1}$ &  & $6.6\!\cdot\!10^{-4}$\\ 
 & 1 & $8.80\!\cdot\!10^{-4}$ & \scriptsize\texttt{(9.0)}\normalsize & $8.8\!\cdot\!10^{-4}$ & $8.37\!\cdot\!10^{-4}$ & \scriptsize\texttt{(9.3)}\normalsize & $1.2\!\cdot\!10^{-4}$ & $8.49\!\cdot\!10^{-4}$ & \scriptsize\texttt{(9.3)}\normalsize & $1.4\!\cdot\!10^{-6}$\\ 
 & 2 & $1.50\!\cdot\!10^{-5}$ & \scriptsize\texttt{(5.9)}\normalsize & $5.1\!\cdot\!10^{-6}$ & $1.53\!\cdot\!10^{-5}$ & \scriptsize\texttt{(5.8)}\normalsize & $4.6\!\cdot\!10^{-7}$ & $1.53\!\cdot\!10^{-5}$ & \scriptsize\texttt{(5.8)}\normalsize & $4.3\!\cdot\!10^{-9}$\\ 
 & 3 & $3.03\!\cdot\!10^{-7}$ & \scriptsize\texttt{(5.6)}\normalsize & $1.9\!\cdot\!10^{-7}$ & $2.99\!\cdot\!10^{-7}$ & \scriptsize\texttt{(5.7)}\normalsize & $2.0\!\cdot\!10^{-8}$ & $3.01\!\cdot\!10^{-7}$ & \scriptsize\texttt{(5.7)}\normalsize & $2.1\!\cdot\!10^{-10}$\\ 
 & 4 & $8.70\!\cdot\!10^{-9}$ & \scriptsize\texttt{(5.1)}\normalsize & $2.0\!\cdot\!10^{-9}$ & $8.51\!\cdot\!10^{-9}$ & \scriptsize\texttt{(5.1)}\normalsize & $4.3\!\cdot\!10^{-10}$ & $8.48\!\cdot\!10^{-9}$ & \scriptsize\texttt{(5.1)}\normalsize & $5.9\!\cdot\!10^{-12}$\\ 
 & 5 & $2.20\!\cdot\!10^{-10}$ & \scriptsize\texttt{(5.3)}\normalsize & $3.1\!\cdot\!10^{-11}$ & $2.18\!\cdot\!10^{-10}$ & \scriptsize\texttt{(5.3)}\normalsize & $7.1\!\cdot\!10^{-12}$ & $2.18\!\cdot\!10^{-10}$ & \scriptsize\texttt{(5.3)}\normalsize & $9.4\!\cdot\!10^{-14}$\\ 


==> num_exp/comp_tableK_k5.tex <==
5 & 0 & $5.67\!\cdot\!10^{-1}$ &  & $4.6\!\cdot\!10^{-3}$ & $5.20\!\cdot\!10^{-1}$ &  & $8.4\!\cdot\!10^{-2}$ & $5.60\!\cdot\!10^{-1}$ &  & $1.2\!\cdot\!10^{-3}$\\ 
 & 1 & $8.61\!\cdot\!10^{-4}$ & \scriptsize\texttt{(9.4)}\normalsize & $3.7\!\cdot\!10^{-4}$ & $8.81\!\cdot\!10^{-4}$ & \scriptsize\texttt{(9.2)}\normalsize & $6.1\!\cdot\!10^{-5}$ & $8.89\!\cdot\!10^{-4}$ & \scriptsize\texttt{(9.3)}\normalsize & $6.9\!\cdot\!10^{-7}$\\ 
 & 2 & $5.39\!\cdot\!10^{-6}$ & \scriptsize\texttt{(7.3)}\normalsize & $4.1\!\cdot\!10^{-7}$ & $5.43\!\cdot\!10^{-6}$ & \scriptsize\texttt{(7.3)}\normalsize & $4.9\!\cdot\!10^{-8}$ & $5.43\!\cdot\!10^{-6}$ & \scriptsize\texttt{(7.4)}\normalsize & $4.8\!\cdot\!10^{-10}$\\ 
 & 3 & $3.55\!\cdot\!10^{-8}$ & \scriptsize\texttt{(7.2)}\normalsize & $7.8\!\cdot\!10^{-9}$ & $3.35\!\cdot\!10^{-8}$ & \scriptsize\texttt{(7.3)}\normalsize & $3.9\!\cdot\!10^{-10}$ & $3.35\!\cdot\!10^{-8}$ & \scriptsize\texttt{(7.3)}\normalsize & $5.5\!\cdot\!10^{-12}$\\ 
 & 4 & $4.36\!\cdot\!10^{-10}$ & \scriptsize\texttt{(6.3)}\normalsize & $1.3\!\cdot\!10^{-10}$ & $4.68\!\cdot\!10^{-10}$ & \scriptsize\texttt{(6.2)}\normalsize & $8.1\!\cdot\!10^{-12}$ & $4.70\!\cdot\!10^{-10}$ & \scriptsize\texttt{(6.2)}\normalsize & $9.3\!\cdot\!10^{-14}$\\ 


==> num_exp/comp_tableSB_k1.tex <==
1 & 0 & $5.09\!\cdot\!10^{-1}$ & $2.06\!\cdot\!10^{-1}$ &  & $5.09\!\cdot\!10^{-1}$ & $2.06\!\cdot\!10^{-1}$ &  & $5.09\!\cdot\!10^{-1}$ & $2.06\!\cdot\!10^{-1}$ & \\ 
 & 1 & $1.57\!\cdot\!10^{-1}$ & $8.07\!\cdot\!10^{-2}$ & \scriptsize\texttt{(1.4)}\normalsize & $1.57\!\cdot\!10^{-1}$ & $8.07\!\cdot\!10^{-2}$ & \scriptsize\texttt{(1.4)}\normalsize & $1.57\!\cdot\!10^{-1}$ & $8.07\!\cdot\!10^{-2}$ & \scriptsize\texttt{(1.4)}\normalsize \\ 
 & 2 & $4.10\!\cdot\!10^{-2}$ & $1.89\!\cdot\!10^{-2}$ & \scriptsize\texttt{(2.1)}\normalsize & $4.10\!\cdot\!10^{-2}$ & $1.89\!\cdot\!10^{-2}$ & \scriptsize\texttt{(2.1)}\normalsize & $4.10\!\cdot\!10^{-2}$ & $1.89\!\cdot\!10^{-2}$ & \scriptsize\texttt{(2.1)}\normalsize \\ 
 & 3 & $9.63\!\cdot\!10^{-3}$ & $4.64\!\cdot\!10^{-3}$ & \scriptsize\texttt{(2.0)}\normalsize & $9.63\!\cdot\!10^{-3}$ & $4.64\!\cdot\!10^{-3}$ & \scriptsize\texttt{(2.0)}\normalsize & $9.63\!\cdot\!10^{-3}$ & $4.64\!\cdot\!10^{-3}$ & \scriptsize\texttt{(2.0)}\normalsize \\ 
 & 4 & $2.37\!\cdot\!10^{-3}$ & $1.13\!\cdot\!10^{-3}$ & \scriptsize\texttt{(2.0)}\normalsize & $2.37\!\cdot\!10^{-3}$ & $1.13\!\cdot\!10^{-3}$ & \scriptsize\texttt{(2.0)}\normalsize & $2.37\!\cdot\!10^{-3}$ & $1.13\!\cdot\!10^{-3}$ & \scriptsize\texttt{(2.0)}\normalsize \\ 
 & 5 & $5.90\!\cdot\!10^{-4}$ & $2.82\!\cdot\!10^{-4}$ & \scriptsize\texttt{(2.0)}\normalsize & $5.90\!\cdot\!10^{-4}$ & $2.82\!\cdot\!10^{-4}$ & \scriptsize\texttt{(2.0)}\normalsize & $5.90\!\cdot\!10^{-4}$ & $2.82\!\cdot\!10^{-4}$ & \scriptsize\texttt{(2.0)}\normalsize \\ 
 & 6 & $1.47\!\cdot\!10^{-4}$ & $7.04\!\cdot\!10^{-5}$ & \scriptsize\texttt{(2.0)}\normalsize & $1.47\!\cdot\!10^{-4}$ & $7.04\!\cdot\!10^{-5}$ & \scriptsize\texttt{(2.0)}\normalsize & $1.47\!\cdot\!10^{-4}$ & $7.04\!\cdot\!10^{-5}$ & \scriptsize\texttt{(2.0)}\normalsize \\ 


==> num_exp/comp_tableSB_k3.tex <==
3 & 0 & $6.59\!\cdot\!10^{-2}$ & $3.54\!\cdot\!10^{-2}$ &  & $8.78\!\cdot\!10^{-2}$ & $4.29\!\cdot\!10^{-2}$ &  & $1.04\!\cdot\!10^{-1}$ & $5.55\!\cdot\!10^{-2}$ & \\ 
 & 1 & $7.44\!\cdot\!10^{-3}$ & $3.60\!\cdot\!10^{-3}$ & \scriptsize\texttt{(3.3)}\normalsize & $2.06\!\cdot\!10^{-2}$ & $8.13\!\cdot\!10^{-3}$ & \scriptsize\texttt{(2.4)}\normalsize & $1.73\!\cdot\!10^{-2}$ & $9.22\!\cdot\!10^{-3}$ & \scriptsize\texttt{(2.6)}\normalsize \\ 
 & 2 & $2.60\!\cdot\!10^{-4}$ & $8.77\!\cdot\!10^{-5}$ & \scriptsize\texttt{(5.4)}\normalsize & $1.46\!\cdot\!10^{-3}$ & $9.22\!\cdot\!10^{-4}$ & \scriptsize\texttt{(3.1)}\normalsize & $1.98\!\cdot\!10^{-3}$ & $6.37\!\cdot\!10^{-4}$ & \scriptsize\texttt{(3.9)}\normalsize \\ 
 & 3 & $8.16\!\cdot\!10^{-6}$ & $2.98\!\cdot\!10^{-6}$ & \scriptsize\texttt{(4.9)}\normalsize & $1.54\!\cdot\!10^{-4}$ & $4.56\!\cdot\!10^{-5}$ & \scriptsize\texttt{(4.3)}\normalsize & $1.41\!\cdot\!10^{-5}$ & $5.45\!\cdot\!10^{-6}$ & \scriptsize\texttt{(6.9)}\normalsize \\ 
 & 4 & $3.53\!\cdot\!10^{-7}$ & $1.47\!\cdot\!10^{-7}$ & \scriptsize\texttt{(4.3)}\normalsize & $1.40\!\cdot\!10^{-6}$ & $5.70\!\cdot\!10^{-7}$ & \scriptsize\texttt{(6.3)}\normalsize & $6.59\!\cdot\!10^{-7}$ & $2.70\!\cdot\!10^{-7}$ & \scriptsize\texttt{(4.3)}\normalsize \\ 
 & 5 & $1.87\!\cdot\!10^{-8}$ & $7.51\!\cdot\!10^{-9}$ & \scriptsize\texttt{(4.3)}\normalsize & $6.93\!\cdot\!10^{-8}$ & $2.75\!\cdot\!10^{-8}$ & \scriptsize\texttt{(4.4)}\normalsize & $3.28\!\cdot\!10^{-8}$ & $1.36\!\cdot\!10^{-8}$ & \scriptsize\texttt{(4.3)}\normalsize \\ 


==> num_exp/comp_tableSB_k4_p10.tex <==
4 & 0 & $6.09\!\cdot\!10^{-1}$ & $3.09\!\cdot\!10^{-1}$ &  & $7.36\!\cdot\!10^{-2}$ & $3.73\!\cdot\!10^{-2}$ &  & $8.69\!\cdot\!10^{-2}$ & $5.67\!\cdot\!10^{-2}$ & \\ 
 & 1 & $7.00\!\cdot\!10^{-3}$ & $2.81\!\cdot\!10^{-3}$ & \scriptsize\texttt{(6.8)}\normalsize & $4.37\!\cdot\!10^{-2}$ & $1.40\!\cdot\!10^{-2}$ & \scriptsize\texttt{(1.4)}\normalsize & $2.32\!\cdot\!10^{-2}$ & $1.36\!\cdot\!10^{-2}$ & \scriptsize\texttt{(2.1)}\normalsize \\ 
 & 2 & $2.16\!\cdot\!10^{-4}$ & $8.17\!\cdot\!10^{-5}$ & \scriptsize\texttt{(5.1)}\normalsize & $6.34\!\cdot\!10^{-3}$ & $2.96\!\cdot\!10^{-3}$ & \scriptsize\texttt{(2.2)}\normalsize & $2.12\!\cdot\!10^{-3}$ & $5.47\!\cdot\!10^{-4}$ & \scriptsize\texttt{(4.6)}\normalsize \\ 
 & 3 & $2.16\!\cdot\!10^{-6}$ & $6.06\!\cdot\!10^{-7}$ & \scriptsize\texttt{(7.1)}\normalsize & $5.07\!\cdot\!10^{-4}$ & $1.31\!\cdot\!10^{-4}$ & \scriptsize\texttt{(4.5)}\normalsize & $9.06\!\cdot\!10^{-6}$ & $3.94\!\cdot\!10^{-6}$ & \scriptsize\texttt{(7.1)}\normalsize \\ 
 & 4 & $4.29\!\cdot\!10^{-8}$ & $1.24\!\cdot\!10^{-8}$ & \scriptsize\texttt{(5.6)}\normalsize & $1.24\!\cdot\!10^{-6}$ & $4.81\!\cdot\!10^{-7}$ & \scriptsize\texttt{(8.1)}\normalsize & $3.41\!\cdot\!10^{-7}$ & $1.48\!\cdot\!10^{-7}$ & \scriptsize\texttt{(4.7)}\normalsize \\ 
 & 5 & $1.29\!\cdot\!10^{-9}$ & $3.75\!\cdot\!10^{-10}$ & \scriptsize\texttt{(5.1)}\normalsize & $5.44\!\cdot\!10^{-8}$ & $2.09\!\cdot\!10^{-8}$ & \scriptsize\texttt{(4.5)}\normalsize & $1.07\!\cdot\!10^{-8}$ & $4.77\!\cdot\!10^{-9}$ & \scriptsize\texttt{(5.0)}\normalsize \\ 


==> num_exp/comp_tableSB_k5.tex <==
5 & 0 & $3.81\!\cdot\!10^{-2}$ & $1.44\!\cdot\!10^{-2}$ &  & $6.46\!\cdot\!10^{-2}$ & $2.73\!\cdot\!10^{-2}$ &  & $9.12\!\cdot\!10^{-2}$ & $4.29\!\cdot\!10^{-2}$ & \\ 
 & 1 & $1.33\!\cdot\!10^{-3}$ & $6.35\!\cdot\!10^{-4}$ & \scriptsize\texttt{(4.5)}\normalsize & $1.49\!\cdot\!10^{-2}$ & $6.27\!\cdot\!10^{-3}$ & \scriptsize\texttt{(2.1)}\normalsize & $1.33\!\cdot\!10^{-2}$ & $6.17\!\cdot\!10^{-3}$ & \scriptsize\texttt{(2.8)}\normalsize \\ 
 & 2 & $3.86\!\cdot\!10^{-5}$ & $1.31\!\cdot\!10^{-5}$ & \scriptsize\texttt{(5.6)}\normalsize & $2.19\!\cdot\!10^{-3}$ & $8.27\!\cdot\!10^{-4}$ & \scriptsize\texttt{(2.9)}\normalsize & $7.02\!\cdot\!10^{-4}$ & $2.74\!\cdot\!10^{-4}$ & \scriptsize\texttt{(4.5)}\normalsize \\ 
 & 3 & $6.08\!\cdot\!10^{-8}$ & $1.49\!\cdot\!10^{-8}$ & \scriptsize\texttt{(9.8)}\normalsize & $9.66\!\cdot\!10^{-5}$ & $2.92\!\cdot\!10^{-5}$ & \scriptsize\texttt{(4.8)}\normalsize & $1.81\!\cdot\!10^{-6}$ & $6.25\!\cdot\!10^{-7}$ & \scriptsize\texttt{(8.8)}\normalsize \\ 
 & 4 & $3.09\!\cdot\!10^{-10}$ & $7.90\!\cdot\!10^{-11}$ & \scriptsize\texttt{(7.6)}\normalsize & $2.20\!\cdot\!10^{-7}$ & $8.83\!\cdot\!10^{-8}$ & \scriptsize\texttt{(8.4)}\normalsize & $3.84\!\cdot\!10^{-8}$ & $1.61\!\cdot\!10^{-8}$ & \scriptsize\texttt{(5.3)}\normalsize \\ 

